CoordX: Accelerating Implicit Neural Representation with a Split MLP Architecture

Implicit neural representations with multi-layer perceptrons (MLPs) have recently gained prominence for a wide variety of tasks such as novel view synthesis and 3D object representation and rendering. However, a significant challenge with these representations is that both training and inference with an MLP over a large number of input coordinates to learn and represent an image, video, or 3D object, require large amounts of computation and incur long processing times. In this work, we aim to accelerate inference and training of coordinate-based MLPs for implicit neural representations by proposing a new split MLP architecture, CoordX. With CoordX, the initial layers are split to learn each dimension of the input coordinates separately. The intermediate features are then fused by the last layers to generate the learned signal at the corresponding coordinate point. This significantly reduces the amount of computation required and leads to large speedups in training and inference, while achieving similar accuracy as the baseline MLP. This approach thus aims at first learning functions that are a decomposition of the original signal and then fusing them to generate the learned signal. Our proposed architecture can be generally used for many implicit neural representation tasks with no additional memory overheads. We demonstrate a speedup of up to 2.92x compared to the baseline model for image, video, and 3D shape representation and rendering tasks.

==> background.tex <==
\section{Background and Motivation}\label{bg_mt}
As an alternative to the explicit representations, coordinate-based MLP can represent the signal at an arbitrary resolution, not bounded by the memory requirement of storing voxels in a typical explicit representation, and it is end-to-end differentiable.

% $\bullet$ 
\textbf{Overview} 
Coordinate-based MLP typically takes an input of low-level spatial or spatial-temporal coordinates and are trained to learn a signal that represent shape or appearance at the coordinate location. For 2D image reconstruction task for example, we model the network as $f_{\theta}: R^n \to R^m$, where $n=2$ is the 2D image pixel $(x,y)$ coordinates, and $m=3$ is the RGB colour at that pixel coordinate location $(x,y)$. To enable MLP to well learn the high-frequency components inside the signals, positional encoding (PE) \citep{mildenhall2020nerf} and sinusoidal activation (SIREN) \citep{sitzmann2020implicit} are the two commonly used techniques. 
Positional encoding maps input coordinate to a higher dimension, which enables the model to learn high frequency details of the scene. The encoding formula can be described as:
\begin{equation}
\gamma(p) = (\sin(2^0\pi p),\cos(2^0\pi p),...,\sin(2^{n-1}\pi p),\cos(2^{n-1}\pi p))
\end{equation}
Where $p$ is the coordinate value for each channel in the input, assuming we want to project coordinate input that is in dimension $\mathbb{R}^m$ to $\mathbb{R}^{2n}$.\\
Sinusoidal activation replaces activation function in MLPs that are piecewise linear (ReLU with its second derivative being zero) to periodic activation functions:
\begin{equation}
    \mathbf{h}_{i} = \sin(\mathbf{W}_i\mathbf{h}_{i-1}+\mathbf{b}_i)
\end{equation}
Where $\mathbf{W}_i,\mathbf{b}_i$ is the weight matrix and bias applied to the input $\mathbf{h}_{i-1}$. To guarantee SIREN MLP be able to converge, a special parameter initialization is also proposed by \cite{sitzmann2020implicit}. Commonly, PE and SIREN are not used together in existing works. 

% $\bullet$ 
\textbf{The training of coordMLP} 
The training of coordMLP start with sampling the coordinate input for the signal that we want to learn. For example, if we are trying to fit a 2D image, we will try to sample points on the image with their 2D coordinates, and there are various sampling strategies such as random sampling or sample in image patches, and many more. Then the coordMLP predicts the signal at the coordinate and calculate the loss with ground truth signal.

% $\bullet$ 
\textbf{Limitation} 
After introducing the coordinate-based MLP, we know that grids of coordinate points are processed by MLP before we can view the signal representation. Unlike CNN, coordMLP treat each coordinate point as a separate input, which results in the extremely large batches of data to be inferred for the actual representation. For 
example,  to display a single image of size $1024\times1024$ represented by a 5-layer coordMLP, we need to do 1,048,576 MLP queries, which takes about 0.2 seconds on one GTX1080 GPU. To render a novel view image of size $400\times400$ with original NeRF model\footnote{8-layer MLP and hierarchical sampling with 64+128 sample points along each ray.}, 30,720,000 query points need to be processed by MLP, which takes about 18 seconds on One GTX1080 GPU, let alone the medium- or large-size rendered images. 
The NeRF model training is also time-consuming because it has dense points to be sampled via ray-casting process for back-propagation optimization. It takes more than 10 hours on RTX Titan to over-fit a synthetic \textit{Lego} scene. The over-fitting nature, a NeRF MLP is fitted to only represent a particular scene, also makes the cost of using NeRF very high
%\footnote{Generalizable NeRF model is still an active research topic but beyond the scope of our work.}. 
From above examples we can see that neural representation with coordMLP is still slow and inefficient when it comes to real-time rendering and some other real-life applications.


% $\bullet$ 
\textbf{Dense, well-aligned data in coordMLP}
When we look at different coordMLP applications, we can easily find that the inference data points of coordMLP are usually dense and well-aligned. Fig. \ref{fig:grids} is an intuitive visualization of coordinate input grids for image, video and 3D shape. These coordinate grids show the very good point alignment which directly inspires our new acceleration method. In the vanilla coordMLPs, each input coordinate point is independent, only responsible for predicting its corresponding signal value. There is no explicit connection in the grids of input points, though some shared information does exist. Take the image grid (Fig.~\ref{grid_img}) for example, points on the same row of pixel grid share the same $y$ coordinate (aligned with $x$-axis), but the same $y$ value combined with $N$ different $x$ values requires $N$ separate queries of coordMLP. On a row of pixel points $[(1,2), (2,2), (3,2), (4,2)]$, $x$ unchanges, $y$ has a slight change each step. There should be overlapping $x$ value related computation inside the MLP for all these points. It works the same way when we look at data aligned with other axes such as $y$, $t$, $z$ on image or other tasks.
%\footnote{NeRF tasks do not have good data alignment due to ray-casting process, we will discuss it later.}. 

If we leverage this observation and propose a new model to take advantage of data alignment, the acceleration of coordMLP is foreseeable, the denser and higher-dimensional the input coordinates are, the more evident the speedup we can achieve.  In the next section, we will discuss our proposed splitting coordMLP that directly uses this observation for the acceleration of neural implicit representation.


==> drafts/experiments.tex <==
\section{Experiments}\label{experiment}
In this section, we validate the benefits of CoordX acceleration with experiments on a variety of signal fitting tasks. In addition, we also make experiments to explore the proper design of CoordX.

\textbf{Setup.} To make the reliable speed and accuracy comparison between normal coordMLP and our CoordX, we choose several existing coordMLP models as our baseline models. We additionally modify or rewrite these baseline models to make them become CoordX models with their corresponding new training and inference pipeline. Specifically, we choose models from SIREN \citep{sitzmann2020implicit} as baseline for image and video representation tasks; we implement 3D occupancy networks following the design from \cite{tancik2020fourier}. Besides, we also test our method on coordMLP with latent codes as a part of the input. In this task, we use a LIIF model from \cite{chen2021learning} as baseline. 
% the nerf result may be put in the appendix.
We use PyTorch \citep{paszke2019pytorch} as the deep learning framework for our experiments, and all the models are trained or tested on one NVIDIA RTX3090.
% The choose the same hyperparameters for our CoordX models as the ones used in corresponding normal coordMLPs.
Unless otherwise specified, most of experiments use 5-layer MLPs, and CoordX models leave two FC layers after fusion operator by default in this case.
CoordX models' other hyperparameters such as learning rate, batch size, number of epochs, etc. are set to be consistent with ones used in corresponding normal coordMLPs. The qualitative demonstrations of these tasks are left at Appendix part.

\subsection{Various Signal Fitting Tasks}

\begin{figure}[tbhp]
%   \vspace{-15pt}
  \centering
  \subfigure[Image inference\label{infer_img} ]{\includegraphics[width=0.37\textwidth]{figs/img_infer_speed.pdf}}
  \subfigure[Video inference\label{infer_video} ]{\includegraphics[width=0.41\textwidth]{figs/viedo_infer_speed.pdf}}
  \subfigure[Shape inference\label{infer_shape} ]{\includegraphics[width=0.208\textwidth]{figs/shape_infer_speed.pdf}}
  \caption{\small Inference speed comparison. PE or SIREN does not show much difference on the inference speed here, so only one set of model configurations is shown here. (a) average time of finishing model inference for a synthetic image for 100 times on different resolutions; (b) million second per frame for representing a synthetic video with 100 frames on different resolutions; (c) time to finish the inference of a grid of coordinate points for marching cubes to display 3D shapes.}
  \label{fig:speed_img_video}
  \vspace{-10pt}
\end{figure}

% \subsubsection{Image Representation}\label{sec:img_recon}
\textbf{Image Representation.}
In this experiment, we use 5-layer coordMLPs with 256 hidden units to fit RGB images of size $512 \times 512$. We randomly select 12 center-cropped images from DIV2K dataset \citep{agustsson2017ntire} to report average PSNR. Table \ref{tab:img_psnr} shows PSNR values and the required training time for 10,000 epochs. In addition, we make an inference speed comparison between normal coordMLP and CoordX on different image sizes based on SIREN models. Fig. \ref{infer_img} shows the testing results. 
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
    Method  & MLP-S  & CoordX-S & CoordX-S-A & MLP-P & CoordX-P & CoordX-P-A \\
    \hline
    PSNR    & %37.50 & 35.93 & 35.75 & 36.36 & 32.46 & 32.71\\
    39.52 & 36.32 & 36.32 & 34.87 & 31.70 & 31.42 \\
    \hline
    Training time & %5.53 & 10.22 & 2.82 & 4.47 & 9.72 & 2.48 \\
    6.03 & 11.17 & 2.87 & 7.40 & 13.90 & 2.53 \\
    \hline
    \end{tabular}
    \caption{Accuracy and speed comparison. MLP indicates the normal coordMLP. S and P refer to SIREN and PE respectively. A refers to accelerated training.}
    \label{tab:img_psnr}
\end{table}

From this experiment, we can see that (i) Our CoordX can achieve high PSNR values that are close to the results from the corresponding normal coordMLPs. The accelerated training in this task has no impact on the final representation quality compared to results from the normal training. (ii) Accelerated training achieves almost two times speedup compared to normal coordMLP's training. (iii) In the inference test, there is an apparent speed gap between normal coordMLP and our CoordX. As we increase the image size, this gap also get larger. Our method can provide near x3 speedup in the large $2048 \times 2048$ inference setting. 

% \subsubsection{Video Representation}\label{exp:video}
\textbf{Video Representation.}
To fit short clips of video with neural implicit representations, we use 5-layer coordMLPs with 1024 hidden units for experiment. We use 2 10-second video clips for this task.

For CoordX models, we consider two splitting strategies here. The first one is to split up height, width and time axes completely, which yields 3 network branches (X+Y+T). The second one is to split up spatial and temporal dimension. Hight and width axes are flattened as one axis in this case, so there are 2 branches in the network (XY+T). PE method is used in this experiment because it has better performance compared to SIREN. Table \ref{tab:video_shape} shows average PSNR values and the required training time for 100,000 epochs. Similar to image representation, we also test inference speed of three models on different frame resolutions. The results are shown in Fig. \ref{infer_video}.

Both X+Y+T and XY+T splitting strategies achieve comparable results. Specifically, XY+T splitting even outperforms baseline model. Accelerated training can provide over 2 times training speedup, while retaining the high representation quality in models without accelerated training. In the inference test, we can observe that two splitting strategies show similar inference speedup because of the frame-by-frame inference. Near near x3 speedup can also be achieved as the frame resolution increases.

\begin{table}[tbph]
\small
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    Task & \multicolumn{4}{c}{Video} & \multicolumn{3}{|c}{3D shape}\\
    \hline
    Method  & MLP  & X+Y+T & XY+T & XY+T-A & MLP & CoordX & CoordX-A\\
    \hline
    Metric    & 33.315 & 31.69 & 33.63 & 33.35 &0.991 / 0.970 & 0.991 / 0.970 & 0.989 / 0.964\\
    \hline
    Training time & 4.30 h & 6.63 h & 5.22 h & 2.13 h & 5.72 min & 16.14 min & 3.28 min \\
    \hline
    \end{tabular}
    \caption{Accuracy and speed comparison. MLP indicates the normal coordMLP. A refers to accelerated training. Video task uses PSNR as the metric, and 3D shape task uses easy / hard IoU (higher is better) as metrics.}
    \label{tab:video_shape}
\end{table}

% \subsubsection{3D Shape Representation}\label{exp:3d_shape}
\textbf{3D shape representation.}
We choose occupancy networks \citep{mescheder2019occupancy} to represent 3D shapes. The networks (coordMLPs) output probabilities to indicate whether points are inside or outside the shape. We use 5-layer coordMLPs with 256 hidden units for this experiment. SIREN method is used here for its better performance.
The used four 3D shapes are selected from The Stanford 3D Scanning Repository\footnote{\url{http://graphics.stanford.edu/data/3Dscanrep/}}. Unlike image and video task, this task uses IoU as the metric. We have two point sets for calculating IoUs: the first set (the easy set) are randomly sampled points inside the object bounding box ; the second set (the hard set) are randomly sampled points around the object surface. Table \ref{tab:video_shape} shows the average IoU values and the required training time for 10,000 epochs. 
To display shapes and compare inference speeds after training, we use the marching cube \citep{lorensen1987marching} process in which a 3D mesh grid of coordinate points are queried. By adjusting the size of the mesh grid, we show the inference speed comparison in Fig. \ref{infer_shape}. 

% Volumetric rendering, as another way to display 3D shapes, will be discussed in Appendix.
% Why volumetric rendering depends solely on grid resolution with non-split architecture and why it also depends on image resolution for split architecture. Explain the advantage of using split architecture in this case (less memory usage for storing feature grid).
We can see that the IoU scores from our models are almost the same as ones from normal coordMLPs. 
Besides, the new sampling strategy used in our accelerated training helps CoordX models achieve 1.7 times training speedup with little accuracy drop.
When it comes to inference speed, our CoordX shows its superiority again.  We can observe more than 2x speedup on two resolution grids, and as the resolution become higher ($256^3$), almost 3x speedup can be achieved. 

% Short conclusion here.
From the results of above three experiments, we can 
draw conclusions that 
(i) CoordX models can generally achieve high representation quality that is comparable to normal CoordMLPs on many tasks, and for CoordX's small quality drop on some dense signal fitting tasks, we will continue the analysis in \ref{coordx_capacity}.
% we will keep discussing the representation quality in section.
(ii) CoordX's inference acceleration is effective, and gets more obvious as the resolution of signal becomes larger. And we can widely see 2.5x or even higher speedup of CoordX's accelerated inference and training, which also justifies our speedup analysis in \ref{sec:speedup}. 
(iii) CoordX's training without acceleration takes longer time than normal CoordMLP's training, while our purposed accelerated training (\ref{accelerated_training}) can make CoordX's training faster than normal CoordMLP's training with a little accuracy drop.



\subsection{Split Method with Latent Codes}\label{image_code}
In this part, we test our CoordX model on more complex coordinate-based MLPs, which include high-dimensional latent codes as part of model inputs for better generalizability. The model we accelerate is LIIF (Local Implicit Image Function) \citep{chen2021learning} for image super-resolution. It takes an 2D pixel position and a high-dimensional LIIF latent code from a CNN encoder as inputs and then predicts the RGB value at the given pixel coordinate. The coordMLP (decoder) here is also a 5-layer MLP with 256 hidden units. We modify the coordMLP part of this big model and design a CoordX model with 4 branches (code,x,y,cell) for this task, where cell is an additional 2D input introduced in \cite{chen2021learning} for better performance. We fix the pretrained EDSR \citep{lim2017enhanced} decoder and train our CoordX decoder from scratch for 1,000 epochs. The same as \cite{chen2021learning}, DIV2K dataset \citep{agustsson2017ntire} is used for quantitative comparison. The target image resolutions for this dataset are on the 2K scale.
Table \ref{tab:llif} shows the differences between original LIIF and our modified CoordX LIIF.

From experimental results we can see that CoordX LIIF model can achieve almost the same PSNR values campared in many different settings compared to original baseline model. And the CoordX shows significant inference speedup (almost x3) on 2K image super resolution. Further speedup is also achievable if we re-use relative coordinates for each LIIF cell. In this way, our splitting method can help LIIF model achieve real-time image super-resolution. 
We can also draw a conclusion that our CoordX is compatible with the current advanced CoordMLPs with latent codes for richer representation.

\begin{table}[tbph]
    \small
    \centering
    \begin{tabular}{c|ccc|ccccc|c}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{In-distribution} & \multicolumn{5}{c|}{Out-of-distribution} & \multirow{2}{*}{Speed}\\ \cline{2-9}
    & $\times 2$ & $\times 3$  & $\times 4$  & $\times 6$  & $\times 12$  & $\times 18$  & $\times 24$  & $\times 30$ & \\
    \hline
    EDSR-baseline-LIIF    & 34.67 & 30.96 & 29.00 & 26.75 & 23.71 & 22.17 & 21.18 & 20.48 & 131.03 ms \\
    \hline
    EDSR-CoordX-LIIF  & 34.65 & 30.95 & 28.99 & 26.67 & 23.60 & 22.08 & 21.10 & 20.42 & 45.53 ms \\
    \hline
    \end{tabular}
    \caption{Accuracy and speed comparison between baseline LIIF model and our modified CoordX LIIF model. PSNR is used as quantitative metric. Scores for EDSR-baseline-LIIF are directly imported from LIIF paper. The speed here is the average time to finish processing all images in DIV2K valid set with $\times 2$ setting. }
    \label{tab:llif}
\end{table}

% \subsection{Ablation Study}


% \subsubsection{Different Types of Fusion Operation}

\subsection{The Degree of Splitting for MLP}
We see CoordX model can be partly split or fully split (Sec. \ref{sec:decompose}). In this part, we explore the impact of different degrees of splitting to the CoordX models. We use 3D shape fitting task for experiments. The CoordX models used in \ref{exp:3d_shape} have 2 FC layers after fusion operator. We treat the number layers after fusion as a hyperparameter ($D_f$) to be swept. 
We change the $D_f$ from 0 to 5 for the 5-layer CoordX models used here. Note that when $D_f = 5$ the coordX model becomes a normal coordMLP. 
And to show the efficacy of splitting FC layers before fusion operator, we also consider normal coordMLP with different model depth ($D_{MLP}$) in this experiment.
All the models use accelerated training strategy purposed in \ref{accelerated_training} including $D_f=5$ case. We use $128^3$ grid of coordinate points to test the inference speed.
The test results are listed in Table \ref{tab:split}.

As $D_f$ becomes lower, the IoU score also decreases slowly. We have to admit that normal coordMLP can better fuse coordinate information, but at the cost of longer training time and much longer inference time. On the other hand, CoordX greatly accelerates the speed of coordinate-based MLPs at the cost of very little quality drop. But such drop is generally acceptable and negligible compared to the quality gap between models with PE (SIREN) and without PE (SIREN). 
In addition, compared to $D_f$-layer normal coordMLP,  our CoordX models gives higher accuracy with very low extra computation, which shows the necessity of splitting FC layers in our models.
Therefore, our method gives the developer enough space to adjust the balance in the trade-off between representation quality and speed.

\begin{table}[htbp]
    % \small
    \centering
    \begin{tabular}{c|cccccc|ccc}
    \hline
    \multirow{2}{*}{Model setting} & \multicolumn{6}{c|}{$D_f$} & \multicolumn{3}{c}{$D_{MLP}$} \\ \cline{2-10} 
    & 5*  & 4 & 3 & 2 & 1 & 0 & 4 & 3 & 2\\
    \hline
    IoU    & 0.976 & 0.980 & 0.974 & 0.963 & 0.941 & 0.880 & 0.959 & 0.876 & 0.516\\
    \hline
    Training time & 5.72 & 5.40 & 4.24 & 3.28 & 2.27 & 2.38 & 4.44 & 3.11 & 1.67  \\
    \hline
    Inference speed & 105.22 & 95.43 & 69.37 & 46.25 & 19.73 & 22.18 & 82.12 & 55.21 & 30.77  \\
    \hline
    \end{tabular}
    \caption{Accuracy and speed comparison. The time unit for training time is minute (min), and the time unit for inference speed is millisecond (ms).
    When $D_f=5$, the CoordX model becomes a normal CoordMLP.}
    \label{tab:split}
\end{table}

\subsection{The Representation Capacity of CoordX}\label{coordx_capacity}
Experimental results above have shown good speed performance of our CoordX models on various tasks. However, we should also notice that CoordX models have slight representation quality drop on image fitting task. We can see from Table \ref{tab:img_psnr} that CoordX models have 2-3 points PSNR drop. While in other tasks, CoordX has much smaller quality gaps and sometimes CoordX even outperforms normal CoordMLP with one exception X+Y+T CoordX on video representation. When we carefully observe these models and tasks, we can find that quality drop mainly comes from representing images with X+Y splitting on 2D image/pixel space. These 2D image signals are much denser (more high-frequency components) compared to other types of signals. 
For example, video can be treated as a mixture of spatial (pixel frame) and temporal (frame id) signals. Compared to spatial signals, temporal signals looks sparser because of high signal continuity in a sequence of consecutive video frames. The dense signals in 2D pixel space require more information fusion from height (X) and width (Y) dimensions for neural nets to well fit, which makes our results in \ref{exp:video} reasonable that XY+T splitting outperforms X+Y+T splitting. Besides, proper decomposition of signals such as XY+T splitting can help improve the representation quality. 3D shapes as another type of signals in our experiment are relatively sparse in 3D space, because signal (occupancy or SDF) changes happen mainly around the surface of a shape.

Now that we see the some limitations of CoordX's representation on dense signals like image, we then explore how to improve CoordX's representation. Recall our analysis in \ref{sec:decompose} about feature decomposition. Our current CoordX only use $R=1$ to approximate the hidden feature tensor. If we can increase the reduction dimension $R$ for more effective fusion, the representation quality should be increased. To increase $R$, we have to add extra parameters in CoordX models for outputting larger branch feature size. But according to our speedup analysis in \ref{sec:speedup}, there still be the chance for our CoordX model to be faster than original normal coordMLP even if more parameters are added to CoordX. 
We consider 2 ways to design the augmented CoordX models: (i) the number of hidden units in the layer right before fusion are multiplied by $R$; (ii) each splitting layer before fusion is $R$ times as large as the original. Apparently, the second way introduces more parameters for fusion, we can expect more quality improvement from this method compared to the first one.  
And naturally, the advantage of second method is the limited extra parameter addition, so that model can still maintain a relatively small size.

We choose SIREN-based models for this experiment. Most of experimental settings are consistent with \ref{sec:img_recon} except that all models are trained for 20,000 epochs for well converged results. We test $R=2$ and $R=3$ for CoordX combined with aforementioned 2 augmentation designs. We only run accelerated training for CoordX models. Table \ref{tab:aug_fusion} shows the performance comparison of different model configurations. 

\begin{table}[htbp]
    \small
    \centering
    % \begin{tabular}{c|c|c|c|c|c|c}
    \begin{tabularx}{36em}%
    {{>{\centering\arraybackslash}p{9em}}*{6}{|>{\centering\arraybackslash}X}}
    \hline
    Model & MLP & CoordX & R2\texttt{+} & R2\texttt{++} & R3\texttt{+} & R3\texttt{++} \\
    \hline
    PSNR    & 40.25 & 37.08 & 39.70 & 41.32 & 41.60 & 43.55  \\
    \hline
    Training time (min) & 12.60 & 5.87 & 7.67 & 7.87 & 9.00 & 9.33  \\
    \hline
    Inference speed (ms) & 52.45 & 22.34 & 29.24 & 34.92 & 30.05 & 37.73 \\
    \hline
    Model size (MB) & 0.77 & 0.77 & 1.02 & 2.27 & 1.27 & 4.78 \\
    \hline
    \end{tabularx}
    \caption{
    Image fitting model comparison. RX means $R=\text{X}$, "\texttt{+}" represents the first augmentation method, while "\texttt{++}" represents the second augmentation method which adds more parameters. The inference speed is the average time to infer a synthetic 1024x1024 image for 100 times.}
    \label{tab:aug_fusion}
\end{table}

We can see from the results that increasing the reduction dimension $R$ successfully improves the representation quality. The augmented CoordX models are now able to achieve higher scores than the baseline normal coordMLPs.
Even though more parameters are added to augmented CoordX models, the training and inference speeds are still faster than the baseline coordMLP.
The second augmentation design (\texttt{++}) can help models get higher scores but at the cost of much larger model size.
Here are some conclusions we can draw from this experiment:
(i) higher $R$ can help models better reconstruct the dense signals when the same model design are kept;
(ii) more extra parameters can help models get better features for fusion when $R$ is unchanged;
(iii) the reduction dimension $R$ plays a more important role than the model size (see R2\texttt{++} vs. R3\texttt{+}).
To sum up, by tuning an additional hyperparameter $R$, our CoordX model can enlarge its representation capacity and get higher fitting scores, while still maintaining high training and inference speed.

% When  we comprehensively look at these augmented models, we can find the reduction dimension $R$ plays a more important role than the model size. For example, in the comparison between R2\texttt{++} and R3\texttt{+}, more extra parameters do not help R2\texttt{++} outperform R3\texttt{+}. Instead, R3\texttt{+} model has higher PSNR and faster inference speed.

% \subsubsection{The Representation Capacity of Split Method}
% Now that CoordX models have shown good performance on various tasks, we want to explore the limit of our representation method in this part. We will use CoordX model to represent some very large and complex images to see the representations' qualitative difference between normal coordMLP and our CoordX.

% We conduct an experiment using 2 images, both having various resolutions ranging from $2,000\times2,000$ to $8,000\times8,000$ pixels, in order to test the limit for coordX model to reach the same accuracy as the original model. We also test our model's ability to represent signals with different level of complexities, therefore one image has relatively low number of features on the image, mainly a pure colored background, while the other image has a high number of features, and have very complex structures. 
% % We find the gigapixel experiment in the work \citep{martel2021acorn} provide us two images fit for this experiment. 
% % For the simple image, we use the Pluto image captured by New Horizon space probe, and we use a panorama picture of Tokyo by Trevor Dobson to represent the complex image.
% % Both image are center-cropped and down-sampled to various resolutions described above. 
% The same as the image task in \ref{sec:img_recon}, 5-layer SIREN MLPs with 256 hidden units are used. Each model is trained for 10,000 epochs.

% As shown in Figure \ref{fig:capacity_graph}, CoordX's performance is close to a normal coordMLP on images with various resolutions. As the resolution gets higher, the PSNR difference with the original model stays relatively constant. While for the SSIM score, CoordX's performance can be worse when resolution goes higher, but when the resolution goes high enough, both models hit a bottleneck as the number of parameters cannot adequately represent such large images, therefore performance difference between the two models become smaller again. As for different complexities, we can also see the performance difference gets larger when image has more 
% information and are more structurally complex.

% Higher SSIM score difference between the two models with higher resolutions can be attributed to the difference between the calculation of PSNR and SSIM. As studies have shown, SSIM are more sensitive to structural content of the image than PSNR, various structural degradation can yield the same results for PSNR and MSE but different for SSIM\citep{wang2009mean}. In our experiment, we found that disentangling coordinates can cause image to have some vertical line distortions, which might not be discriminated by PSNR but can cause SSIM to drop.

% \begin{figure}[tbhp]
%   \centering
%   \subfigure[PSNR Comparison for simple image\label{simple_psnr} ]{\includegraphics[width=0.45\textwidth]{figs/simple_psnr.pdf}}
%   \subfigure[PSNR Comparison for complex image\label{complex_psnr} ]{\includegraphics[width=0.45\textwidth]{figs/complex_psnr.pdf}}
%   \subfigure[SSIM Comparison for simple image\label{simple_ssim} ]{\includegraphics[width=0.45\textwidth]{figs/simple_ssim.pdf}}
%   \subfigure[SSIM Comparison for complex image\label{complex_ssim} ]{\includegraphics[width=0.45\textwidth]{figs/complex_ssim.pdf}}
%   \caption{Qualitative comparison between normal coordMLP (MLP) and CoordX (Ours) on high resolution images, PSNR (above) and SSIM (below) on different image complexities. 1k, 2k, 4k, 8k each stands for $1000 \times 1000$, $2000 \times 2000$, $4000 \times 4000$, $8000 \times 8000$ image resolutions.}
%   \label{fig:capacity_graph}
% \end{figure}

% \begin{table}[htbp]
% \small
% \centering
% \begin{tabular}{c|cc|cc|cc|cc} 
% \hline
% Task       & \multicolumn{4}{c|}{Complex}                        & \multicolumn{4}{c}{Simple}                          \\ 
% \hline
% Method     & \multicolumn{2}{c|}{MLP} & \multicolumn{2}{c|}{Ours} & \multicolumn{2}{c|}{MLP} & \multicolumn{2}{c}{Ours}  \\ 
% \hline
% Resolution & 1k & 2k                  & 1k & 2k                  & 1k & 2k                  & 1k & 2k                  \\ 
% \hline
% PSNR       & 25.62  & 22.52                   & 23.56  & 20.22                   & 29.90  & 26.40                   & 28.69  & 25.34                   \\ 
% \hline
% SSIM       & 0.7465  & 0.6411                   & 0.5640  & 0.4451                   & 0.8483  & 0.7466                   & 0.7646  & 0.6446                   \\
% \hline

% \end{tabular}
% \caption{Qualitative comparison for image representation on high resolution. MLP indicates the normal coordMLP.}
% \label{tab:capacity}
% \end{table}

==> drafts/introduction_v0.tex <==
\section{Introduction}
 Implicit neural representation have been a main interest in recent research, especially with the coordinate-based multilayer perceptrons (MLP), aiming to replace the traditional discrete representations for a variety of high-frequency low-dimensional signals like images and shapes.

$\bullet$ Brief intro what is coordinate-based MLP.\\
As its name suggests, coordinate-based MLP (coordMLP) is a type of neural network that takes low dimensional coordinates (e.g., position or time index) as input and predicts the signal value (e.g., color, depth, shape, etc.) of each corresponding coordinate point. As implicit functions, this type of networks learns a continuous mapping between coordinates and signal values, via the gradient based supervised optimization.

$\bullet$ Brief discussion about what are the advantages of this kind of representation.\\
Comparing with the discrete representations, this type of model is significantly more memory efficient. Unlike the discrete representation where the granularity of the represented object is limited by the grid resolution/point density, the granularity of  this neural implicit representation can be freely adjusted by choosing different resolutions of input coordinates as long as not exceeding the representation capacity of the learned MLP. The fully differentiable optimization process allows MLP to learn the complete signals from sparsely sampled data points e.g., random sampling and ray-casting based sampling.

$\bullet$ List some impressive applications of using this MLP, e.g., \cite{mildenhall2020nerf}, \cite{park2019deepsdf}, \cite{chen2021learning}, etc.\\
Some existing works using CoordMLPs have achieved state-of-the-arts results on a wide range of signal fitting or learning tasks such as image super-resolution \citep{chen2021learning}, 3D shape representation \citep{park2019deepsdf,mescheder2019occupancy,gropp2020implicit}, novel view synthesis \citep{mildenhall2020nerf,martin2021nerf,schwarz2020graf,pumarola2021d} and photo-realistic 3D scene editing \citep{niemeyer2021giraffe}. The impressive results presented in these works well show the power of coordinate-based MLP.

$\bullet$ Point out problems that limit the usage of this new type of representation.\\
However, one coin has two sides. The outstanding application results of coordinate-based MLP are usually at the cost of orders of magnitude higher computation compared to normal methods. It is obvious that the MLP based implicit representation need more computation because of the one-to-one mapping, parameterized as a MLP, between coordinate points and representing signal values (Sec. \ref{bg_mt}). 
% For example, one 2,000$\times$1,000 image has $2,000,000$ pixel points to be inferred via the MLP. 
Densely sampled coordinate points usually require a huge amount of computation even though the neural network is just a shallow MLP. In addition to that, this unique feature also makes the training of coordMLP very time-consuming.

$\bullet$ And our goal in this works is to accelerate training and inference of coordMLPs while retaining accuracy as much as possible.

$\bullet$ What do prior work do in this space? And why does it not solve the problem?\\
The compute-intensive nature of coordMLP is also noticed by other researchers. There are some existing works trying to improve the speed of coordMLP \citep{liu2020neural, neff2021donerf, takikawa2021neural, garbin2021fastnerf, yu2021plenoctrees, reiser2021kilonerf, martel2021acorn}. Most of these acceleration works specifically focus on novel view synthesis tasks and make use of the spatial sparsity inherent in the 3D objects (Sec. \ref{related}). A common solution in these works is to use explicit-implicit combined representation. Explicit representation first provides the rough surface/point estimation of the object, then coordMLP is charge of the fine-grain object representation. But this solution also has its limitation, i.e., it cannot be easily applied to other types of signals with dense spatial/temporal data. Besides, the introduction of explicit representation also makes this new form of signal representation not that memory-efficient.

$\bullet$ In order to do this, we leverage the observation ..... Summarize a common property of existing applications of coordinate-based MLP. Add a figure for more intuitive explanation. The points on the well-aligned data grids share a lot coordinate information mutually. This is a property neglected by existing works.\\
Unlike prior works, this work finds a completely new direction to accelerate the coordMLP on a variety of signal fitting tasks based on our observation that dense and well-aligned coordinate data are fed into the coordMLP (Sec. \ref{bg_mt}). The points on these well-aligned data grids share a lot coordinate information mutually (Fig. \ref{fig:grids}). This is actually a common property of existing applications of coordMLP, but neglected by most of existing works. 

$\bullet$ Our key idea in this work is .. \\
Based on the aforementioned property, we propose an new idea that makes the computation of coordMLP be more efficient. We first split up coordinate channels and then fuse the features from different channels to avoid a lot of computation for similar low-dimensional coordinate values. % We call our method CoordX as it splits up coordinate input for speedup. 

$\bullet$ What are the issues? Why is it difficult to do this\\
The key issue for our method is how to modify/design a new network architecture in order to take advantage of the dense coordinate alignment in the different tasks while maintaining the high representation accuracy as well as the compact model size shown in original coordMLPs. To make it faster, the corresponding training and inference pipeline may also need modifications. 

$\bullet$ Summarize the key points of our split-MLP.\\
To address this issue, we carefully design three parts of our new MLP--the input layer, layers between input and fusion, fusion operators (Sec. \ref{method}). We call our model \emph{CoordX} as it splits up coordinate input for speedup. CoordX can realize significant training and inference speedup on different signal fitting tasks including image, video, 3d shape fitting tasks. The speedup depends on the size and dimension of input points. More than x2 speedup can be widely achieved in our experiments. In the mean while, with almost no model size changes, CoordX also maintains the high representation accuracy with almost no or minimal accuracy drop compared to the original non-split model. In addition, we also discuss the reason why CoordX works from the aspect of the matrix decomposition. This explanation also shows other potential applications related to matrix decomposition.

To summarize, our contributions include:
\begin{itemize}
    \item A new acceleration direction for coordinate-based MLP by leveraging the dense coordinate alignment commonly shown in different signal fitting applications.
    \item A split MLP architecture design that keeps the model size unchanged but achieve faster training and inference speed with high accuracy; and reasonable analysis of why our model works.
    \item Demostration of CoordX's speedup on various signal fitting tasks including image, video and 3D shape; incorporation of CoordX into other advanced applications such as image super-resolution.
    % , \sout{dynamic noval view synthesis}(\textbf{TODO}).
\end{itemize}，

==> drafts/method_v0.tex <==
\section{Method}\label{method}
We design a new MLP architecture (CoordX) that uses multiple branches for each decomposed part of the original input coordinates to better utilize the inherent coordinate alignment from the input points.
Fig. \ref{fig:network} shows the architecture comparison between normal coordMLP and our CoordX. Details will be discussed in the following subsections.
% Aiming to utilize the dense well-aligned point or coordinate queries to the coordinate-based MLP to achieve acceleration, our work relies on two major parts: (i) a channel-split coordinate-based MLP architecture (CoordX) that splits up the coordinate input of a coordMLP into number of different channels, without changing the number of parameters; (ii) depending on the task for the model, we modify the training process of coordMLP with new data sampling strategies to utilize the split architecture to achieve further acceleration. 

% We expand the dimension to the input coordinates so that during fusion, each new dimension is expanded to match dimension size at that dimension for other feature vectors from other channels. In this case, feature for the first channel that has size $H \times 1 \times M$ is being expanded automatically to $H \times W \times M$, and the feature for the second channel that has size $1 \times W \times M$ is also being expanded  to $H \times W \times M$, so that an element-wise operation can happen.

\subsection{Neural Network Architecture}
%  \textbf{Model Overview}  
Our split network architecture can be divided into three parts: (i) a feature extraction layer for each split coordinate branch; (ii) a set of shared layers outputting split features for each branch; (iii) a fusion operation followed a few FC layers to fuse split features and output final prediction.
% includes a feature extraction layer for each split coordinate branch, a set of shared layers for each branch's features, a fusion operation that merges features from each branch, and a set of final layers after fusion that follows the original design of the normal coordMLP. 
The mapping between coordinates and signals is basically unchanged.
\begin{equation}
    \Phi : \mathbb{R}^{K} \mapsto \mathbb{R}^{O}
\end{equation}
Where $K$ is the input dimension of the coordinate  and $O$ is the dimension of output signal, e.g., $K=2, O=3$ if model learns the image signal.
% \textbf{Coordinate Splitting/Decomposing}



In typical CoordMLP models, a set of $N$ coordinate points are individually queried as inputs (where $N=HW$ for an image of size $H \times W$ in Fig. \ref{fig:normalMLP}). This set of coordinate points, $\mathbf{X}\in\mathbb{R}^{N\times K}$, where $K$ is the dimension of each point (e.g., $K=2$ for $(x,y)$ points on a pixel plane), can form a $C$-dimensional  grid of size $B_i\times\cdots\times B_C$, e.g., $N$ image coordinate points for image form a $H\times W$ grid ($C=2,B_1=H,B_2=W$) in Fig. \ref{fig:coordsplit1}, coordinate values inside each point directly tells its location on the grid.
After reshaping the points into the grid, we can find that only a subset of $K_i$ positions in the $K$-D coordinate change for points along $i$th axes, thus $\mathbf{X}$ can be decomposed into $C$ parts. Each part $\mathbf{X}^{(i)}$ has the shape $B_i\times K_i$ ($\sum_i^CK_i = K$). 
% , where $K_i$ is the size of the subset of coordinate positions that changes along $i$th axis.
For example, points on 2D image (Fig. \ref{fig:coordsplit1}) can be decomposed into 2 parts (Fig. \ref{fig:coordsplit2}\&\ref{fig:coordsplit3}): the first part $\mathbf{X}^{(1)}$ containing the position $x$ of 2D $(x,y)$ coordinate, as the value of $x$ only changes along the vertical axis of length $H$; the second part containing the position $y$, as $y$ only changes along the horizontal axis of length $W$. Note that $K_i$ sometimes can be larger than one (or $C<K$), e.g., 3D video points $(x,y,t)$ ($K=3$) can also form a $C=2$ dimensional grid. The two decomposed parts then contain the position $(x,y)$ and $(t)$ respectively.


























Base on the coordinate alignment of corresponding signal fitting task, one $K$-D input point $\mathbf{x} \in \mathbb{R}^{K}$ from the coordinate grid $\mathbf{X}$ can be split up into $C$ parts $\{\mathbf{x}^{(i)}| i=1,2,\dots,C\}$, where $\mathbf{x}^{(i)} \in \mathbb{R}^{K_i}$ and $\sum_i^CK_i = K$. Note that $C$ may be smaller than $K$, e.g., 
% video fitting task in \ref{exp:video} and image with latent codes in \ref{image_code}). 
if positional encoding (PE) is used, the input we split up becomes the encoded input and $K_i$ in this case is much larger than 1. These split sub-coordinates then becomes the input to our model.
% Because commonly used PE and SIREN method do not change the fact that coordinate inputs are dense and well-aligned, PE/SIREN can be well incorporated into our split model CoordX, and most of our experimental results in Sec. \ref{experiment} actually use PE or SIREN as part of CoordX model. 

\textbf{First layer} 
% splitting up the weights to get 2 branches of FC layers. Two channels going through two separate layers.
% 
% To begin with, assume the original model has the first layer as follows\footnote{We omit the bias term $\mathbf{b}$ in the following equations for simplicity.}:
% \begin{equation}
% \label{eq:ori}
%     \mathbf{h}_1 =\phi (\mathbf{W}_1\mathbf{x})
% \end{equation}
% Where $\mathbf{W}_1 \in \mathbb{R}^{M \times K}$ is the weight matrix, and $\mathbf{h}_1 \in \mathbb{R}^{M}$ is the extracted feature output from the first layer. $M$ is the number of hidden features for this layer. $\phi(\cdot)$ is the activation function.
% As the coordinate input $\mathbf{x}$ has been split up into $C$ parts, 
The first layer of our split coordMLP contains $C$ parallel branches for corresponding $\mathbf{x}^{(i)}$. Accordingly, the weight matrix $\mathbf{W}_1\in \mathbb{R}^{M \times K}$ is split up into $C$ sub-matrices $\{\mathbf{W}_1^{(i)}, i=1,2,\dots,C\}$, where $\mathbf{W}_1^{(i)}\in \mathbb{R}^{M \times K_i}$. 
In this way, we change first layer's formulation into: %\ref{eq:ori} into:
\begin{equation}\label{eq:firstlayer}
    % \mathbf{h}_1 \rightarrow
    \{\mathbf{h}_1^{(i)}=\phi(\mathbf{W}_1^{(i)}\mathbf{x}^{(i)})| i=1,2,\dots,C\}
\end{equation}
\textbf{Layers before fusion} % \textbf{Layers between first and fusion}
% After the first layer, we get features for each separated branch $\mathbf{h}_1^{(i)} \in \mathbb{R}^{M}$.
Since we do not want to add additional parameters to our model, we use the shared weight matrices (FC layers) to process hidden features from all parallel branches after the first layer (Fig. \ref{fig:network}). Suppose there are $D_s$ layers before fusion, we can formulate these layers as:
\begin{equation}
    \{\mathbf{h}_j^{(i)}=\phi(\mathbf{W}_j\mathbf{h}_{j-1}^{(i)})| i=1,2,\dots,C\},\quad {j = 2,\dots,D_s}
%    a = \phi(\mathbf{W}_s\mathbf{h}) = \phi(\sum_{i=1}^n \mathbf{W}_s\mathbf{h}_i) \approx \sum_{i=1}^n\phi(\mathbf{W}_s\mathbf{h}_i) 
\end{equation}
% Assuming the original model has its non-first layers formulated as $a = \phi(\mathbf{W}_s\mathbf{h})$, where $a$ is the layer's output, and $\mathbf{W}_s$ is the weight of the layer, and $\mathbf{h}$ is the feature output from the previous layer.\\
Like the convolutional layer in CNN where one kernel extracts features from different sliding windows on the large input, our design of these layers has threefold benefits: (i) no extra parameters are added because of one layer for all branches (weight-sharing); (ii) better computational efficiency/parallelism compared to separate FC layers, because all features can be concatenated and be fed in one batch; (iii) joint optimization with gradients from all branches, which helps layers capture meaningful information from all encoded inputs. 

\textbf{Feature Fusion}
Our CoordX model compose splitting features $\mathbf{h}_{D_s}^{(i)}$ from $C$ branches to to get the fused feature $\mathbf{h}_{D_s}^* \in \mathbb{R}^{M}$.  
The fusion here should be an element-wise operation such as product, summation or an attention layer \citep{vaswani2017attention}. 
% As the preliminary work in splitting coordinate-based MLP,
We choose product as CoordX's fusion operation, because product operation gives a better explanation on splitting mechanism from the aspect of matrix decomposition, which will be discussed in detail in \ref{sec:decompose}. Formally, the fusion operation can be formulated as follows:
\begin{equation}\label{eq:fusion}
    \mathbf{h}_{D_s}^* = \text{Fuse}(\mathbf{h}_{D_s}^{(1)}, \cdots, \mathbf{h}_{D_s}^{(C)}) = \prod_{i=1}^C \mathbf{h}_{D_s}^{(i)}
\end{equation}
Note that Eqn. \ref{eq:firstlayer}-\ref{eq:fusion} only shows the computation for one coordinate input. %from splitting to fusing. 
In real application, a grid of coordinate inputs are fed into network (Fig. \ref{fig:network}). 
The coordinate decomposition (splitting coordinate and removing duplicate values) of the grid generates input vectors (matrices) $\mathbf{X}^{(i)} \in \mathbb{R}^{B_i\times K_i}$ for $C$ split branches, where $B_i$ is the number of sub-coordinate inputs at branch $i$. Accordingly, we have the hidden feature matrices $\mathbf{H}^{(i)}_{D_s} \in \mathbb{R}^{B_i\times M}$ to be fused. And the fusion in this case can be formulated as
\begin{equation}\label{eq:fusion_vec}
    \mathbf{H}_{D_s,p_1p_2\dots p_C}^* = \text{Fuse}(\mathbf{H}_{D_s}^{(1)}, \cdots, \mathbf{H}_{D_s}^{(C)}) = \prod_{i=1}^C \mathbf{H}_{D_s,p_i}^{(i)}
\end{equation}
The fused feature tensor $\mathbf{H}_{D_s}^* \in \mathbb{R}^{B_1\times \cdots\times B_C\times M}$, and $\prod_{i=1}^{c}B_I$ equals to the number points on the input grid $\mathbf{X}$. Eqn. \ref{eq:fusion_vec} can be efficiently computed by modern tensor computing libraries with broadcasting mechanism. We will leave $D_f$ normal FC layers after fusion for further feature fusion and outputting final predicted signals.

\textbf{Speedup Analysis}\label{sec:speedup} After showing the CoordX model's architecture, we can clearly see how CoordX speeds up the coordMLP inference. Suppose we have a coordinate gird with $N = B^C$ points to be inferred by a $D$-layer MLP, normal coordMLP has the batch size of $N=B^C$ for each layer from layer 1 to layer $N$, which results in $\mathcal{O}(DB^C)$ FC layer computation in total, while our CoordX model with $C$ branches can provide more efficient inference, where the first $D_s$ layers before fusion in this case only need to process $C\cdot B$ split inputs each, and the rest $D_f$ layers ($D_s+D_f=D$) process the fused features of the original size $B^C$. The two parts in CoordX result in $\mathcal{O}(D_sCB + D_fB^C)$ FC layer computation in total. 
%The computation gap between normal coordMLP and CoordX $\mathcal{O}\left(D_s(B^C-CB)\right)$  depends on $D_s$, $B$ and $C$ and is usually very large in real applications (high order polynomial increase v.s. linear increase).
The ratio $\gamma$ of the amount of computation between two method is 
\begin{equation}
    \gamma = \frac{(D_s+D_f)B^C}{CD_sB + D_fB^C} = \frac{D_s+D_f}{CD_sB^{1-C}+D_f} = \frac{\lambda + 1}{\lambda CB^{1-C} + 1},\quad\lambda = \frac{D_s}{D_f}
\end{equation}
% talk about slower case?
when $B$ is large enough, the term $\lambda CB^{1-C}$ will become very small and negligible. And we can get a theoretic upper bound for our speedup ratio $\gamma \rightarrow \lambda + 1$. For example, for a commonly used 5-layer MLP, we choose $D_f=2$ to build our CoordX model, then $D_s=3$ and $\lambda = D_s/D_f = 1.5$. We can therefore expect a 2.5x speedup of CoordX model on the inference of dense coordinate grids\footnote{2.5x here is based on the assumption that each FC layer have the same amount of computation.}.




%  \textbf{Activation before/after fusion} 
% % Mention that changing the order of activation and fusion doesn't affect the results that much.
% Alternatively, we can also exchange the order for fusion operation and the layers after first layer, so that we perform fusion first, and then fused features go through the share layers and final layers. But as experiment results shown in \ref{experiment}, changing the order of the two operations doesn't have significant impact on the performance and accuracy of the model.

%  \textbf{Generalization}
% Our model is a modification based on the current coordMLP architecture, and has the exact same number of parameters as the original model. In the first layer when we split up the coordinate input channels and assign them an individual feature extraction layer, we split up the weight parameters for the first layers as well, as shown in Eqn. \ref{eq:firstlayer}, and we did not increase or decrease the number of parameters for layers after the first layer.\\
% Our model is also very generalized, and can adopt common signal representation methods such as positional encoding \citep{mildenhall2020nerf} and SIREN \citep{sitzmann2020implicit}.


% Mention that after our modification the model have same number of parameters as the original model, and that it could adopt common signal representation methods such as positional encoding and sine activation.
% Mention that feeding multiple coordinate channels of features into the same FC layer makes almost no difference when use separate FC layers for each coordinate channel.

\subsection{Split coordinate training acceleration}\label{accelerated_training}
% We have shown how CoordX achieves acceleration by taking advantage of good data-alignment of input coordinates. 
% In this subsection, we show how to accelerate CoordX model training. 
Our CoordX model can work with the original training pipeline without any modification, but no training speedup can be achieved. Because inputs are treated as independent coordinate points in the original training, our CoordX model has to individually process each coordinate point.
Similar to inference, CoordX's training process can be accelerated by reusing computed features from split coordinate input branches. 
But the feature reuse is possible only when the inputs show good coordinate alignment. The original training process does not hold this property because the points in one training batch are randomly sampled in most cases.
To address this problem, we propose a new sampling strategy in which we first randomly sample 1D positions along each of $K$ axes , then combine these 1D positions to get $K$-D coordinates as the final sampled points for training. Our new sampling approach ensures approximately the same number of points are sampled compared to original sampling. More details about our random sampling are shown in Appendix \ref{rand_sample}.

\subsection{The feature/signal decomposition of CoordX.}\label{sec:decompose}
The feasibility of CoordX design can also be explained from the aspect of feature or signal decomposition. Recall that coordMLP, as a explicit coordinate-signal mapping function, tries to fit low-dimensional signal data. These low-dimensional signals themselves are able to be decomposed with some mathematical tools. For example, a gray-scale image can be treated as a 2D matrix. The decomposition of this image is to calculate a certain type of matrix decomposition such as SVD and QR decomposition. 
Now let's get back to split coordMLP for image fitting. Our CoordX model can also be designed to decompose the signal matrix, i.e., we move the fusion operator to the tail of the CoordX and set the number of layers after fusion to be 0 (fully-split CoordX, like the model shown in Fig. \ref{fig:decompose}). After model training, we can see that this CoordX model is also able to well represent the image with PSNR value very close to 40 (the right part of Fig. \ref{fig:decompose}). We can generalize this idea to (i) other types of signals in 2D, 3D or even higher represented by fully-split CoordX; (ii) fused hidden features from vanilla CoordX models with network layers after fusion. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figs/decompose.pdf}
    \caption{CoordX learns the image decomposition. Left: the coordX's architecture. Fusion operator (dot product) directly output predicted signal. $M$ is the size of hidden feature. $M$ is set to be 256 for fitting the image on the right. Right: visualization of image decomposition learned by CoordX. The image can be represented as a matrix multiplication between two learned feature tensors (matrices) $\mathbf{H}_x$ and $\mathbf{H}_y$.}
    \label{fig:decompose}
\end{figure}

Formally, suppose the coordinate inputs $\mathbf{X}$ can be split up into $C$ branches for fusion in CoordX, i.e., $\{\mathbf{X}_i\in\mathbb{R}^{B_i \times K_i}| i=1,2,\dots,C\}$ follow our prior equations.
The each branch's hidden features $\mathbf{H}^{(i)}_{D_s}$ before the fusion are reshaped into $B_i \times M \times R$. $M$ is the output feature or signal dimension, while $R$ is the dimension that will be reduced by dot product. Now we can use these notions to represent the general case of CoordX's decomposition. For example, when we use fully-split coordX to represent a RGB image , then $M=3$ and $R$ can be any length predefined by user (e.g., 256 in Fig. \ref{fig:decompose}); when $\mathbf{H}^{(i)}$ are some intermediate hidden features to be fused, then $M$ is the input feature size of the next network layer, and $R=1$ as we want to keep the model size unchanged. Next, we assume the fusion operation is dot product, then the fused features/signals $\mathbf{H}^*$ can be formulated as 
\begin{equation}
    \mathbf{H}^*_{p_1p_2\cdots p_C,m} = \sum_{i=1}^{R}{\prod_{j=1}^{C}{\mathbf{H}^{(j)}_{p_j,m,i}}}
\end{equation}
In this way, we successfully extend the idea of two-way matrix decomposition into the multi-way tensor decomposition. Our splitting coordMLP tries to learn a coordinate related feature/signal decomposition during the training process. We should note that even though $R=1$ is used to learn the fused hidden features in vanilla CoordX, it still learns good signal representation in the end. This decomposition also benefits from the coordMLP's continuous representation, which makes it easy to be scaled to different resolutions without considering effects of interpolation in traditional methods.
% As a exploratory work, the CoordX's decomposition currently does not show much meaningful information and is more time-consuming compared to composition methods from linear algebra.

==> introduction-old.tex <==
\section{Introduction}
In recent research, implicit neural representation has been a primary interest, especially with the coordinate-based multilayer perceptrons (MLP), which provides a new way to represent and learn various complex high-frequency low-dimensional signals.
% $\bullet$ Brief intro what is coordinate-based MLP.
As its name suggests, coordinate-based MLP (coordMLP) is a type of neural network that takes low dimensional coordinates (e.g., position or time index) as input. It predicts the signal value (e.g., color, depth, shape, etc.) of each corresponding coordinate point. As an implicit function, coordMLP learns a continuous mapping between coordinates and signal values via gradient-based optimization.

% $\bullet$ Brief discussion about what are the advantages of this kind of representation.\\
Compared with the discrete representations, this type of model is significantly more memory efficient. Unlike the discrete representation where the granularity of the represented object is limited by the grid resolution/point density, the granularity of this neural implicit representation can be freely adjusted by choosing different resolutions of input coordinates as long as not exceeding the representation capacity of the learned MLP. The fully differentiable optimization process allows MLP to learn the complex signals from sparsely sampled data points e.g., random sampling and ray-casting based sampling.
% $\bullet$ List some impressive applications of using this MLP, e.g., \cite{mildenhall2020nerf}, \cite{park2019deepsdf}, \cite{chen2021learning}, etc.\\
Some existing works using CoordMLPs have achieved state-of-the-arts results on a wide range of signal fitting or learning tasks such as image super-resolution \citep{chen2021learning}, 3D shape representation \citep{park2019deepsdf,mescheder2019occupancy,gropp2020implicit}, novel view synthesis \citep{mildenhall2020nerf,martin2021nerf,schwarz2020graf,pumarola2021d} and photo-realistic 3D scene editing \citep{niemeyer2021giraffe}. The impressive results presented in these works well show the power of coordinate-based MLP.

% $\bullet$ Point out problems that limit the usage of this new type of representation.\\
However, the outstanding results from coordMLP applications are usually at the cost of orders of magnitude higher computation compared to traditional methods. It is obvious that the MLP based implicit representation need more computation because of the one-to-one mapping, parameterized as a MLP, between coordinate points and represented signal values (Sec. \ref{bg_mt}).
Densely sampled coordinate points usually require a huge amount of computation even though the neural network is just a shallow MLP. In addition to that, this unique feature also makes the training of coordMLP very time-consuming.
And our goal in this work is to accelerate inference and training of coordMLPs while retaining accuracy as much as possible.

% $\bullet$ What do prior work do in this space? And why does it not solve the problem?\\
The compute-intensive nature of coordMLP is also noticed by other researchers. There are some existing works trying to improve the speed of coordMLP \citep{liu2020neural, neff2021donerf, takikawa2021neural, garbin2021fastnerf, yu2021plenoctrees, reiser2021kilonerf, martel2021acorn}. Most of these acceleration works specifically focus on novel view synthesis tasks and make use of the spatial sparsity inherent in the 3D objects (Sec. \ref{related}). A common solution in these works is to use explicit-implicit combined representations. Explicit representation first provides the rough surface/point estimation of the object, then coordMLP is charge of the fine-grain object representation. But this solution also has its limitation, i.e., it cannot be easily applied to other types of signals with dense spatial/temporal data. Besides, the introduction of explicit representation also makes this new form of signal representation not that memory-efficient.

% $\bullet$ In order to do this, we leverage the observation ..... Summarize a common property of existing applications of coordinate-based MLP. Add a figure for more intuitive explanation. The points on the well-aligned data grids share a lot coordinate information mutually. This is a property neglected by existing works.\\
Unlike prior works, this work finds a completely new direction to accelerate the coordMLP on a variety of signal fitting tasks based on our observation that dense and well-aligned coordinate data are fed into the coordMLP (Sec. \ref{bg_mt}). The points on these well-aligned data grids share a lot coordinate information mutually (Fig. \ref{fig:grids}). This is actually a common property in many existing applications of coordMLP, but neglected by most of existing works. 
% $\bullet$ Our key idea in this work is .. \\
Based on the aforementioned property, we propose an new idea that makes the computation of coordMLP more efficient. We first split up coordinate channels and then fuse the features from different channels to avoid a lot of computation for similar low-dimensional split coordinate values.

% $\bullet$ What are the issues? Why is it difficult to do this\\
The key issue for our method is how to modify/design a new network architecture in order to take advantage of the dense coordinate alignment in the different tasks while maintaining the high representation accuracy as well as the compact model size shown in original coordMLPs. To make it faster, the corresponding training and inference pipeline may also need modifications.
% $\bullet$ Summarize the key points of our split-MLP.\\
To address these problems, we carefully design three parts of our new MLP--the input layer, layers between input and fusion, fusion operation (Sec. \ref{method}). 

We call our model \emph{CoordX} as it splits up coordinate input for speedup. CoordX can realize significant training and inference speedup on different signal fitting tasks including image, video, 3d shape fitting tasks. The speedup depends on the size and dimension of input points, and more than x2 speedup can be widely achieved in our experiments. In the mean while, with almost no model size changes, CoordX also maintains the high representation accuracy with almost no or minimal accuracy drop compared to the original non-split model. In addition, we also discuss the reason why CoordX works from the aspect of the matrix decomposition. This explanation also shows other potential applications related to matrix decomposition.

To summarize, our contributions include:
\begin{itemize}
    \item A new acceleration direction for coordinate-based MLP by leveraging the dense coordinate alignment commonly shown in different signal fitting applications.
    \item A split MLP architecture design that keeps the model size unchanged but achieve faster training and inference speed with high accuracy; and reasonable analysis of why our model works.
    \item Demostration of CoordX's speedup on various signal fitting tasks including image, video and 3D shape; incorporation of CoordX into other advanced applications such as image super-resolution.
    % \sout{dynamic noval view synthesis}(\textbf{TODO}).
\end{itemize}

==> main.tex <==
% \documentclass{article}

% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2021

% % ready for submission
% \usepackage[preprint]{neurips_2021}

% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2021}

% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2021}

% % to avoid loading the natbib package, add option nonatbib:
%     % \usepackage[nonatbib]{neurips_2021}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
% \usepackage{amsmath,amssymb,amsfonts, amsthm}
% \usepackage{subfig}
% \usepackage{tabularx}
% \usepackage{caption}
% \usepackage{blindtext}
% \usepackage{graphicx}
% \usepackage{algorithm2e}
% \usepackage{multicol}

% \title{CoordX: Channel-Split Coordinate-based MLPs}

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.

% \author{%
%   Ruofan Liang \\
%   \texttt{ruofan@cs.toronto.edu} \\
%   \And
%   Hongyi Sun\\
%   \texttt{hongyi.sun@mail.utoronto.ca}\\
%   % examples of more authors
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   \AND
%   \textnormal{University of Toronto}
  
% }
% \begin{document}

% \maketitle

% \input{abstract}

% \input{introduction}

% \input{background}

% \input{related_work}

% \input{methodology}

% \input{experiment}

% \input{conclusion}

% \input{ack}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \section*{Checklist}

% % %%% BEGIN INSTRUCTIONS %%%
% % The checklist follows the references.  Please
% % read the checklist guidelines carefully for information on how to answer these
% % questions.  For each question, change the default \answerTODO{} to \answerYes{},
% % \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% % justification to your answer}, either by referencing the appropriate section of
% % your paper or providing a brief inline description.  For example:
% % \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% % \end{itemize}
% % Please do not modify the questions and only use the provided macros for your
% % answers.  Note that the Checklist section does not count towards the page
% % limit.  In your paper, please delete this instructions block and only keep the
% % Checklist section heading above along with the questions/answers below.
% % %%% END INSTRUCTIONS %%%

% % \begin{enumerate}

% % \item For all authors...
% % \begin{enumerate}
% %   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
% %     \answerTODO{}
% %   \item Did you describe the limitations of your work?
% %     \answerTODO{}
% %   \item Did you discuss any potential negative societal impacts of your work?
% %     \answerTODO{}
% %   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
% %     \answerTODO{}
% % \end{enumerate}

% % \item If you are including theoretical results...
% % \begin{enumerate}
% %   \item Did you state the full set of assumptions of all theoretical results?
% %     \answerTODO{}
% % 	\item Did you include complete proofs of all theoretical results?
% %     \answerTODO{}
% % \end{enumerate}

% % \item If you ran experiments...
% % \begin{enumerate}
% %   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
% %     \answerTODO{}
% %   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
% %     \answerTODO{}
% % 	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
% %     \answerTODO{}
% % 	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
% %     \answerTODO{}
% % \end{enumerate}

% % \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% % \begin{enumerate}
% %   \item If your work uses existing assets, did you cite the creators?
% %     \answerTODO{}
% %   \item Did you mention the license of the assets?
% %     \answerTODO{}
% %   \item Did you include any new assets either in the supplemental material or as a URL?
% %     \answerTODO{}
% %   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
% %     \answerTODO{}
% %   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
% %     \answerTODO{}
% % \end{enumerate}

% % \item If you used crowdsourcing or conducted research with human subjects...
% % \begin{enumerate}
% %   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
% %     \answerTODO{}
% %   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
% %     \answerTODO{}
% %   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
% %     \answerTODO{}
% % \end{enumerate}

% % \end{enumerate}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \clearpage
% \bibliographystyle{unsrt}
% \bibliography{ref}

% \appendix

% \input{appendix}

% \end{document}
